Relating Complexity, Explicitness, Effectiveness of Refactorings and Non-Functional Requirements: A Replication Study

Refactoring is a practice widely adopted during software maintenance and evolution. Due to its importance, there is extensive work on the effectiveness of refactoring in achieving code quality. However, developer's intentions are usually overlooked. A more recent area of study involves the concept of self-affirmed refactoring (SAR), where developers explicitly state their intent to refactor. While studies on SAR have made valuable contributions, they provide little insights into refactoring complexity and effectiveness, as well as the refactorings' relations to specific non-functional requirements. A study by Soares et al. addressed such aspects, but it relied on a quite small sample of studied subject systems and refactoring instances. Following the empirical method of replication, we expanded the scope of Soares et al.'s study by doubling the number of projects analyzed and a significantly larger set of validated refactorings (8,408). Our findings only partially align with the original study. We observed that when developers explicitly state their refactoring intent, the resulting changes typically involve a combination of different refactoring types, making them more complex. Additionally, we confirmed that such complex refactorings positively impact code's internal quality attributes. While refactorings aimed at non-functional requirements tend to improve code quality, our findings only partially align with the original study and contradict it in several ways. Notably, SARs often result in fewer negative impacts on internal quality attributes despite their frequent complexity. These insights suggest the importance of simplifying refactorings where possible and explicitly stating their goals, as clear intent helps shape more effective and targeted refactoring strategies.

==> sections/old/03-dataset.tex <==
\subsection{Dataset Design}

In order to build the \datasetName{} dataset, we employed the following steps and procedures:

\subsubsection{Open-Source project selection}

In order to begin building the dataset, we had to first select open-source projects from which we would collect pull request discussions. For that, we utilized the following inclusion criteria: The open-source system (i) has to be hosted on GitHub; (ii) has to utilize a pull-based development workflow; (iii) has to have at least 1k commits and pull-requests; (iv) has to be at least 5 years old; and (v) has to be in active development. 

Additionally, we also only selected projects that are written in Python, Javascript, Typescript or Python. These programming languages were chosen due to them being often employed in different domains. Domain diversity was also a focus when picking individual software projects. 

Utilizing the aforementioned criteria, we selected \datasetSysNum{} projects. The full list of projects selected is available in our replication package \cite{website}. While more projects fulfilled our criteria, we intentionally selected a small number of projects given the highly manual tasks needed to build the dataset. 

\subsubsection{Selecting messages From pull request discussions} 

After selecting the projects, we utilized the GitHub API to collect all messages exchanged in pull request discussions throughout the history of each of the selected projects. This process resulted in the collection of approximately 1 million messages.

Our next step was to select which messages would be manually labeled. For that, since technical messages are often neutral \citetodo{}, we employed a pre-classification step utilizing the SentiStrengthSE tool \citetodo{} (see Section \citetodo{}). Utilizing that tool, we divided the messages into 3 groups, based on their classification (\textit{i.e.,} positive, negative, and neutral). We also filtered messages which were sent by bots. The final selection was done in two rounds. For the first round, 1000 messages from our 12 Java projects were randomly selected (\textit{i.e.}, 350 random positive messages, 350 random negative messages, and 300 random neutral messages). 

After manually classifying the first round of messages (see step 3), we selected a second round of messages. For this round, additional messages was selected from our 24 Python, Javascript, and Typescript projects. Since we identified while classifying the first round of messages that the distribution of our dataset was skewed towards neutral messages, we selected 48 messages (i.e., 20 random positive messages, 20 random negative messages, and 20 random neutral messages) from each of the 24 projects, totaling 1200 messages.

\subsubsection{Manually classifying each message}

\hl{Falar sobre a tripla validação}

\hl{Falar sobre o modelo de emoções}

A Manual sentiment analysis classification was carried out based on \cite{shaver1987}'s theoretical model, taking into consideration the entire context of a given comment, including interactions before and after the comment. In this model, each emotion can be paired with a polarity: positive or negative. 

The concept of neutrality is not defined by this theoretical approach. However, neutral labels have been utilized in previous research \cite{calefato2018icse, murgia2014wcmsr}. These studies established that neutral denotes the absence of emotion. Since this guide takes a dimensional approach to sentiment analysis, our neutral label will encompass both the absence of emotion and the cases in which the difference between the negative and positive scale equals zero. Therefore the final classification will contain "positive", "negative" and “neutral” polarities. 

\subsubsection{Discussing the disagreements}

During the previous step, we identified several messages where the 3 validators disagreed regarding their classification (i.e., they each classified the message as neutral, positive, and negative, respectively). This totaled $\approx$3\% (\hl{N}) of the 2200 messages. In these cases, we asked the validators to discuss the message and reach an agreement. The results from those discussions were included as the final classifications for the dataset.

\subsubsection{Excluding messages from the dataset}

While we took some steps to remove invalid messages from our sample (\textit{e.g.}, filtering messages from bots), we identified several messages which should be removed from the dataset during the manual classification. Therefore, we employed the following criteria after the classification to exclude messages from the dataset: (i) messages with no textual content (\textit{e.g.}, only mentions, links, etc.), except for emojis; (ii) messages written by bots; (iii) messages not in english; and (iv) duplicated messages. 

\subsection{Dataset Description}

==> tasks.tex <==

1) Pre-processamento dos dados = Coutinho

2) Rodar as ferramentas (total 5) 
DEVA >> João Victor
Senti4SD >> Breno
SentiCR >> Johny \& Breno
2 tools >> Coutinho

3) Revisar Introdução \& Backgroud= Juliana
   Melhorias Background = Luisa, Bia, e Maria Vitória

4) Criação de uma figura de overview = 
Luisa 
Paulo 

5) Seção 2 = nova seção sobre ferramentas (verificar citações)
DEVA >> João Victor
Senti4SD >> Breno
SentiCR >> Johny \& Breno
SentiStrength e SentiStrengthSE >> Vinícius

6) Seção 3 = Coutinho \& Juliana

7) Seção 6 = Coutinho

